Investigating Software Developers' Challenges for Android Permissions in Stack Overflow

The Android permission system is a set of controls to regulate access to sensitive data and platform resources (e.g., camera). The fast evolving nature of Android permissions, coupled with inadequate documentation, results in numerous challenges for third-party developers. This study investigates the permission-related challenges developers face and the solutions provided to resolve them on the crowdsourcing platform Stack Overflow. We conducted qualitative and quantitative analyses on 3,327 permission-related questions and 3,271 corresponding answers. Our study found that most questions are related to non-evolving SDK permissions that remain constant across various Android versions, which emphasizes the lack of documentation. We classify developers' challenges into several categories: Documentation-Related, Problems with Dependencies, Debugging, Conceptual Understanding, and Implementation Issues. We further divided these categories into 12 subcategories, nine sub-subcategories, and nine sub-sub-subcategories. Our analysis shows that developers infrequently identify the restriction type or protection level of permissions, and when they do, their descriptions often contradict Google's official documentation. Our study indicates the need for clear, consistent documentation to guide the use of permissions and reduce developer misunderstanding leading to potential misuse of Android permission. These insights from this study can inform strategies and guidelines for permission issues. Future studies should explore the effectiveness of Stack Overflow solutions to form best practices and develop tools to address these problems.

==> old/1-background.tex <==
\section{Background}
Android permissions are to create a secured system that limits access to sensitive data and privileged components, ensuring only authorized entities can access them. Since Android 9, Android has started restricting permissions to limit non-SDK permissions' usage ~\cite{gorski2019acminer}. There are four official categories \footnote{https://developer.android.com/reference/android/Manifest.permission}:
\begin{itemize}
\item SDK (whitelist) includes supported and documented permissions. In addition, the SDKs which are documented in the package index are specifically called public-API rest are whitelisted. 
\item Blocklist (blacklist) inaccessible by third-party developers.
\item Conditionally Blocked (greylist-max-x) allows access to permission and corresponding interfaces by apps targeting an API level up until level x but is inaccessible for others.
\item Unsupported (greylist) includes those that are unrestricted at the time of publishing but not included in the documentation, therefore, subject to changes without notice.
The non-SDK permissions consist of the permissions which are Blocklisted, Conditionally Blocked, and Unsupported. These non-SDK permissions are not officially documented. 
\end{itemize}

==> old/3-methodology_old.tex <==
\section{Methodology}

\subsection{Goal and Research Questions}
The goal of this study is to identify the common challenges related to evolving permissions faced by Android developers and explore the solutions by the Android community to address these challenges. To achieve our goal, we posed four research questions: 


\textbf{RQ1: What are the specific restrictions types and protection levels of permissions tend to cause the most issues for developers?}

As permissions have different restriction types and protection levels. In some cases the restriction types evolve over versions. he aim of this research question is to explore which types of restrictions and levels of protection are more likely to pose challenges for developers. Additionally, it seeks to understand whether developers encounter more issues with permissions that change over time, or those that remain constant.


\textbf{RQ2: What are the common challenges developers encounter while using evolving permissions?}
    
This research question investigates common challenges developers encounter with evolving permissions, focusing on complexities in adapting to updates, maintaining compatibility, and ensuring security across diverse devices and Android versions. 

\textbf{RQ3: What are the common solutions provided by the community to address the permission-related challenges? }
    
Through this research question, we aim to identify the prevalent solutions proposed by the community to tackle permission-related issues. The inquiry focuses on understanding the strategies and best practices recommended by developers, users, and experts in addressing challenges related to permissions management, ensuring proper protection levels, and mitigating potential risks associated with granting permissions to applications. We grouped the solutions proposed to solve the challenges into some key categories. 

\textbf{RQ4: Is the community providing the correct information about the restriction type and protection level of the permissions? }
    
With this research question, we are investigating whether the community accurately conveys information regarding the restriction type and protection level of permissions. This inquiry seeks to determine if the shared knowledge accurately represents the constraints and safety measures associated with various permissions, ensuring that users and developers clearly understand the implications of granting specific permissions to applications. 



\subsection{Study Design}
The study design, including the data extraction, processing, and analysis (steps 1-9), is depicted in Figure ~\ref{fig:studydesign}.
 \circled{1} We extracted SO posts from the archive called Stack Exchange data dump\footnote{https://archive.org/details/stackexchange}. \circled{2} We filtered out the posts from August 2018 (Android restrictions introduction) to October 2022. \circled{3} We extracted permissions and the corresponding categorization in the Android non-SDK restriction lists published by Google for Android 10, 11, 12, and 13. This resulted in 765 unique permissions. \circled{4} We analyzed the extracted permissions for each Android version and determined which permissions transitioned to different restriction categories across Android versions. For our analysis, we selected  permissions that evolved from one restriction type to another, and this yielded 63 permissions. %\NS{this has to be justified now, because we started with a different goal in mind}. 
\circled{5} We mapped the selected permissions to the SO post's title and body content and initially found 1534 posts related to our selected permissions. %\NS{how it resulted? what was removed?} 
These posts included discussions regarding 43 permissions. \circled{6} We removed duplicate posts and posts with broken links, leaving us with 1216 posts.  We also removed the posts that mentioned specific Android permission in the post's title or body but had issues unrelated to permissions. Our final set included 1,074 posts (summarized in Table ~\ref{table:datasummary}) relating to 43 permissions. \circled{7}  The collected posts were parsed to remove the special characters, XML notations, and emojis. 
Then, we performed qualitative analysis for categorization (\circled{8}) and quantitative analysis to determine the distribution of the posts by Android version and restriction type, frequency of the posts without solutions, and the distribution of the categorized challenges addressed by different solutions categories (\circled{9}).

\begin{figure}[htp]
    \centering
    \includegraphics[width= 8.75 cm]{permission.png}
    \caption{Study Design}
    \label{fig:studydesign}
\vspace{-10pt}
\end{figure}

%\NS{the figure 1 should be revised - > use the circles to it is easier to match description to figure, should be plural: posts, lists, note that step 4 is gone, so relabel everything}

\subsection{Data Analysis}
Our collected data included posts regarding different versions of Android. For further analysis, we categorized the posts as \textit{version-specific posts} and \textit{version non-specific posts} based on whether Android version information was provided. 

\begin{table}[]
\begin{tabular}{lrrr}
\hline
Data Source  & \multicolumn{1}{l}{\# Total} & \multicolumn{1}{l}{\# Filtered} & \multicolumn{1}{l}{\# Analyzed} \\ \hline
\begin{tabular}[c]{@{}l@{}}SO Posts\end{tabular} & 1,399,295 & 1,216 & 1,074 \\ 
\begin{tabular}[c]{@{}l@{}}Permissions\end{tabular} & 765 & 63 & 43  \\ \hline
\end{tabular}
\caption {Summary of Dataset}
\label{table:datasummary} 
\vspace{-30pt}
\end{table}

Out of the total 1074 posts, 501 specified an Android version, and  573  did not. Among 501 \textit{version-specified posts}, the vast majority (401) were related to public and SDK permissions, i.e., \textit{POST\_NOTIFICATIONS, BLUETOOTH\_SCAN, READ\_MEDIA\_VIDEO} were documented and allowed for use by third-party developers. 11 posts were related to blocked permissions, indicating that they were not open for use in third-party apps. Lastly, 34 posts were related to conditionally blocked permissions. Interestingly, all the posts related to conditionally blocked permissions were for Android 10, and the permissions were greylist-max-o. 
%\NS{check what conditional block 34 permissions had}
%\NS{you added permissions examples, I asked you to check what cond. block they had, were they all max-o?}
However, 56 posts (referred to as  \textit{Unmatched} henceforth) included references to permissions that did not exist for a specific Android version in the post. This analysis is summarized in Table ~\ref{table:version_wise_restriction}.
%We created a group called \textit{Unmatched}, which consists of posts that mention but the corresponding permission is not in that version's permission list. 

To address RQ1, the collected posts were analyzed in two steps. First, we performed open coding to identify the themes, patterns, and concepts. Open coding is a qualitative research method used to analyze data in an exploratory and iterative way ~\cite{glaser2016open}. Second, based on the findings from open coding, we categorized the challenges faced by developers. One author performed open coding on the 1074 posts. They went through the dataset, identified patterns, and assigned codes to represent the concepts that emerged from the data. Another author then participated in a verification process. With a 95\% confidence level and a 5\% margin of error, we randomly sampled 292 posts. They independently reviewed the sample of the coded data to ensure the codes accurately reflected the data. Any discrepancies or differences in coding were discussed and resolved through a consensus-building process. This verification step helped to increase the reliability and validity of the analysis, as it ensured that the coding process was consistent and reliable across all coders. This qualitative analysis derived five main categories: \textit{Documentation, Development, Configuration, Security, and Privacy}. These were further divided into subcategories as in Figure~\ref{fig:classification_questions}. We provided descriptions and examples for all categories in the replication package\footref{fn:rp}. %Figure ~\ref{fig:classification} provides the summary of this categorization.  

\begin{figure*}[h]
    \centering
    \includegraphics[width= 15 cm]{categorigation_question_study_01.png}
    \caption{Categorization of Questions Corresponding to Challenges (WS= With Solution, W/OS = Without Solution)}
    \label{fig:classification_questions}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width= 10 cm]{categorization_answers_study1.png}
    \caption{Categorization of Answers Corresponding to Provided Solutions (WS= With Solution, W/OS = Without Solution)}
    \label{fig:classification_answers}
\end{figure*} 
%\NS{change this figure: Stack Oveeflow Posts, remove 'guideline': should be permission implement., feature implem., for errors: error due to Android evol. should be rephrased - not clear what you're implying, the rest: incorrectly implem., other errors }

To address RQ2, we extracted 1107 solutions for the 1074 posts. Similar to the analysis of RQ1, we used open coding and grouped the solutions into three major categories, summarized in Table ~\ref{table:Solution}.
Each post has two scenarios: either it had solutions to the challenge mentioned in it or no solution. 757 posts have solutions to the challenges, and 317 do not. We can also have one or multiple solutions for the challenges. We created four categories for the post containing solutions: \textit{one solution, two solutions, three solutions, and more than three solutions}, as depicted in Table ~\ref{table:number_of_solution}. The summary is presented in the replication package\footref{fn:rp}. 

% Then, we calculated the average number of solutions per challenge in each challenge categories of challenges. 

%We conducted quantitative data analysis and computed and compared various metrics, such as the total number of challenges, the number of challenges with, the number of challenges without answers, and the minimum, maximum, and average number of answers for each sub-group and the overall group. 

\begin{table}[]
\scalebox{.7}{
\begin{tabular}{lrrrrrr}
\hline
\multicolumn{1}{c}{Android} & \multicolumn{6}{c}{Permission Restriction Categories} \\
\multicolumn{1}{c}{Version}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\#Public-\\ API\end{tabular}} & \multicolumn{1}{c}{\#SDK} & \multicolumn{1}{c}{\#Blocked} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\#Conditionally\\ Blocked\end{tabular}} & \multicolumn{1}{c}{\#Greylist} & \multicolumn{1}{l}{Unmatched}  \\ \hline
10  & - & - & - & 34 & 1  & 27 \\ 
11 & 166  & 16  & 11  & - & -  & 29 \\ 
12  & 174 & 22  & -  & -  & - & -  \\ 
13 & 39 & 3 & - & -  & -  & -  \\ \hline
Total & 362  & 39  & 11  & 34  & 1 & 56 \\ \hline
\end{tabular}
}
\caption{\label{table:version_wise_restriction} Summary of the Version-Specific Posts}
\vspace{-15pt}
\end{table}


\begin{table}[]
\scalebox{0.9}{
\begin{tabular}{lrrr}
\hline
& \multicolumn{3}{c}{\#Solutions}\\ 
\multicolumn{1}{c}{Posts Categories} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Related to\\ Documentation\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Development \\ Guideline\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Required\\ Configuration\end{tabular}} \\ \hline
Documentation & 25 & 108 & 75 \\
Configuration & 11 & 55 & 42 \\
Development & 90 & 341 & 347 \\
Security & 1 & 2 & 3 \\
Privacy & 0 & 3 & 3 \\ \hline
\multicolumn{1}{l}{Total} & \multicolumn{1}{r}{127} & \multicolumn{1}{r}{509} & \multicolumn{1}{r}{470} \\ \hline
\end{tabular}}
\caption{\label{table:Solution} Categorization of Posts Corresponding to Solutions}
\vspace{-15pt}
\end{table}

%\NS{Oishwee, you're not using word challenges correctly, most times you refer to issues face by developers or posts, so change where appropriate, e.g., tables, table captions}\\
%\NS{also all your posts are permission-related, so indicating this every time (" Permission Related Challenges") does not make sense}

\begin{table}[]
\begin{tabular}{lrrrrr}
\hline
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Posts \\Categories \end{tabular}} & 
\multicolumn{1}{l}{\#1-S} & \multicolumn{1}{c}{\#2-S} & \multicolumn{1}{c}{\#3-S} & \multicolumn{1}{c}{\#>3-S} & Average \\ \hline
Documentation & 98 & 15 & 8 & 8 & 1.17 \\
Configuration & 54 & 15 & 5 & 2 & 1.02 \\ 
Development & 408 & 71 & 40 & 23 & 0.99 \\ 
Security & 4 & 1 & 0 & 0 & 1.20 \\ 
Privacy & 2 & 1 & 0 & 0 & 1.20 \\ \hline
Total & \multicolumn{1}{l}{568} & 104 & 55 & 26 &  - \\ \hline
\end{tabular}
\caption{\label{table:number_of_solution} Summary of Solutions (1-S = 1 solution, 2-S = 2-solutions, 3-S = 3-solutions, >3-S = more than 3 Solution)}
\vspace{-20pt}
\end{table}

==> old/4-result_old.tex <==
\section{Results}
\textbf{Challenges [RQ1]} The five main categories for the developers' challenges are depicted in Figure ~\ref{fig:classification} and reported next.

%\NS{should be rewritten to give an explanation, simply listing of numbers is not useful, numbers are already in a table, e.g., :}
\textbf{Development} 
The majority of the posts fall in the \textit {Development} category (781), i.e., seeking guidance on the implementation. 
Most of these posts were related to developers looking for help (714 in \textit{Seeking Implementation Guideline} subcategory) or for a solution to resolve existing errors (\textit{Permission Specific Error} subcategory with 67 posts). 
For \textit{Seeking for Implementation Guideline}, we identified 321 posts regarding guidelines for permission implementation in their apps (\textit{Permission Implemention}), 386 posts asked for \textit{Feature Implementation} guideline, and seven posts were investigating how to reproduce a permission-related crash (\textit{Crash Reproduction}). 
The subcategory \textit{Permission Specific Error} refers to permissions not providing desired behaviors or permission causing error in an app (67 posts). The subcategories include \textit{Absence of Required Permission}, which are errors due to the absence of required permissions (43 posts), \textit{Errors with Runtime Permission} - errors related to runtime permissions (3 posts), \textit{Google Rejects Sensitive Permissions} - 
Google rejects the app due to usage of sensitive permissions (16 posts), \textit{Other Permission Specific Error} includes other permission-specific errors which do not fall in any of the above-mentioned types of errors (5 posts).

\textbf{Documentation} 
The second most popular challenges pertain to \textit {Documentation}, which includes 174 posts, i.e., posts requiring help to interpret or find official documentation to implement the app. These posts are further divided into four subcategories: 
\textit{Lack of Documentation} relates to the absence of sufficient or comprehensive information about permission (43 posts),  
\textit{Confusing Documentation} regarding official documentation that was challenging to understand, unclear, and with incomplete descriptions (110 posts),
\textit{Contradictory Documentation} referring to situations when various sources of the Android platform's documentation provide inconsistent information on how to implement a certain feature or how a specific method, API, or permission acts (8 posts), and
\textit{Following Documentation Causes Error} concerning errors caused when developers followed the official documentation (17 posts).

\textbf{Configuration}
This category refers to the settings and parameters necessary for an app to result in the desired behavior (105 posts). Among these posts, 87 were related to \textit{Device/Version/Language Specific Problem}, and 18 were regarding issues where permissions depend on other components such as package, method, library, module, SDK or API-level (SDK or API-level express the application's compatibility with one or more versions of the Android platform) categorized as \textit{Dependency}.

\textbf{Security} 
Only five posts pertained to developers seeking guidance on best practices for secure coding, up-to-date latest security features, and mechanisms provided by Google.

\textbf{Privacy} 
Similarly, five posts refer to the application's problem-related privacy feature and privacy-friendly best practices. For example, \textit{``how to use more privacy friendly best practices, such as Storage Access Framework or Media Store API."}

Next, we report on the permissions' restriction type related to the challenges. We found that out of the 1074 posts, 501 mentioned a version, while more than half of the posts (573) did not. As in Table ~\ref{table:version_wise_restriction}, among the 501 version-specific posts, 362 mentioned Public-API permissions-related challenges, 34 posts were related to Conditionally Blocked, 11 posts were related to Blocked, and one was related to Greylisted permissions.

\begin{comment}
\NS{I still see challenges everywhere}
\textbf{Challenges Categorization [RQ1]} 
We divided the challenges into five categories (with quantity in parentheses): \textit {Documentation} (\#174),  \textit {Configuration} (\#100),  \textit{Development} (\#792),  \textit{Privacy} (\#3), and  \textit{Security} (\#5). These are depicted in green in Figure ~\ref{fig:classification} and further broken down into nine subcategories, seven sub-subcategories, and three sub-sub-subcategories except security and privacy.

\textbf{Development:} The \textit{Documentation} category was further divided into four subcategories: \textit{Lack of  Documentation} (\#43), \textit{Confusing Documentation} (\#108),  \textit{Contradictory Documentation} (\#8), and  \textit {Following Documentation Causes Error} (\#15). 

\textbf{Configuration: }The \textit {Configuration} category had two subcategories: \textit{Dependency} (\#15) and \textit{Device / Version / Language Specific Problem} (\#85). 

\textbf{Development:} This category had the highest number of issues and was divided into two subcategories: \textit{Error} (\#269), \textit{Seeking for Implementation Guideline} (\#523). Then \textbf{Error} subcategory was further divided into four sub-subgroups: \textit{Error due to Android Evolution} (\#135), \textit{Permission Specific Error} (\#73), \textit{Wrongly Implemented Class/Method/Library} (\#36), and \textit{Other Error} (\#25). Next, \textbf{Permission Specific Error} sub-subcategory had four sub-sub-subcategories: \textit{Absence of Required Permission} (\#32), \textit{Runtime Permission} (\#3), \textit{Google Rejects for Sensitive Permission} (\#16), and \textit{Other Permission Specific Error} (\#22). Lastly, the \textbf{Seeking for Implementation Guideline} subcategory had three specific sub-subcategories: \textit{Permission Specific Guideline} (\#277), \textit{Feature Implementation Guideline} (\#239), and \textit{Crash Reproduction} (\#7). 
The descriptions and examples for all categories and subcategories in the replication package\footnote{https://bit.ly/3YHmwiH}.


\end{comment}
\textit{Summary RQ1: Overall, we identified five core categories, nine subcategories, seven sub-subcategories, and three sub-sub-subcategories. Half of the posts did not mention any version. However, when an Android version was mentioned, most of the challenges were related to public API permissions.}


\textbf{Solutions [RQ2]}
317 of 1074 posts did not have a solution. For the remaining 757 posts, we extracted 1106 solutions for the 1074 posts. 
We categorized the solutions as follows: \textit{Development Guideline, Solutions from Documentation, and Suggested Required Configuration.} 
As summarized in Table ~\ref{table:Solution}, 127 solutions referred to documentation or an explanation of the documentation (\textit{Solutions from Documentation}),
509 solutions provided implementation guidelines (\textit{Development Guideline}), and 470 suggested proper configuration for implementing a feature, using permission, or solving an error (\textit{Suggested Required Configuration}). As depicted in Table ~\ref{table:number_of_solution}, over half of the posts (568) have one solution, and only 26 posts have more than three solutions.

\textit{Summary RQ2: Our analysis uncovered three high-level categories for the solutions to the challenges. 317 posts had no solutions, and most posts had one solution.}

==> old/prev_meth_result.tex <==
\section{Methodology}

\subsection{Goal and Research Questions}
The goal of this study is to identify the common challenges related to evolving permissions faced by Android developers and explore the solutions by the Android community to address these challenges. To achieve our goal, we posed four research questions: 


\textbf{RQ1: What are the specific restrictions types and protection levels of permissions tend to cause the most issues for developers?}

As permissions have different restriction types and protection levels. In some cases the restriction types evolve over versions. The aim of this research question is to explore which types of restrictions and levels of protection are more likely to pose challenges for developers. Additionally, it seeks to understand whether developers encounter more issues with permissions that change over time, or those that remain constant.

\textbf{RQ2: What are the common challenges developers encounter while using permissions?}
    
This research question investigates common challenges developers encounter with permissions, focusing on complexities in adapting to updates, maintaining compatibility, and ensuring security across diverse devices and Android versions. 

\textbf{RQ3: What are the common solutions provided by the community to address the permission-related challenges? }
    
Through this research question, we aim to identify the prevalent solutions proposed by the community to tackle permission-related issues. The inquiry focuses on understanding the strategies and best practices recommended by developers, users, and experts in addressing challenges related to permissions management, ensuring proper protection levels, and mitigating potential risks associated with granting permissions to applications. We grouped the solutions proposed to solve the challenges into some key categories. 

\textbf{RQ4: Is the community providing the correct information about the restriction type and protection level of the permissions? }
    
With this research question, we are investigating whether the community accurately conveys information regarding the restriction type and protection level of permissions. This inquiry seeks to determine if the shared knowledge accurately represents the constraints and safety measures associated with various permissions, ensuring that users and developers clearly understand the implications of granting specific permissions to applications. 


\subsection{Study Design}

The study design, including the data extraction, processing, and analysis (steps 1-10), is depicted in Figure ~\ref{fig:studydesign}.

In step \textcircled{1}, we extracted SO posts from the archive called Stack Exchange data dump\footnote{https://archive.org/details/stackexchange}. Next, in step \textcircled{2}, we filtered out the questions from August 2018 (Android restrictions introduction) to October 2022. We extracted permissions and the corresponding categorization of the restriction type and protection level published by Google for Android 10, 11, 12, and 13 in step \textcircled{3}. For restriction type, we extracted the permissions and restriction type from Android's official site \footnote{https://developer.android.com/guide/app-compatibility/restrictions-non-sdk-interfaces}. For the protection level, we extracted the permissions and its' protection level from the source code of Android 13 main branch. In step \textcircled{4}, we took the unique permissions from both extracted permission lists and resulted in 766 permissions (summarized in Table ~\ref{table:permissionsummary}). 

\begin{table}[H]
\scalebox{.63}{
\centering
\begin{tabular}{lrrrrr} 
\hline
Source & \begin{tabular}[c]{@{}l@{}}Android 9/10 \\Permission List\end{tabular} & \begin{tabular}[c]{@{}l@{}}Android 11\\Permission List\end{tabular} & \begin{tabular}[c]{@{}l@{}}Android 12\\Permission List\end{tabular} & \begin{tabular}[c]{@{}l@{}}Android 13 \\Permission List\end{tabular} & \begin{tabular}[c]{@{}l@{}}Android 13 \\Source Code\end{tabular} \\ 
\hline
\# Permission & 533 & 589 & 690 & 765 & 752 \\
\hline
\end{tabular}}
\caption{Permissions Extraction Summary}
\label{table:permissionsummary} 
\end{table}

In the next step (\textcircled{5}), we extracted questions with Android permission-related tags (<android>, <permissions>, <android-permissions>). As there is no previous research mentioning the android permission related tags and there might be some incorrectly tagged permission related questions. To include those questions in our dataset in step \textcircled{6}, we mapped the permissions to the SO question's title and body content and initially found 3128 questions related to permissions.  In this step, we extracted 2021 questions. We realized that there are questions with the permissions named: BACKUP, DUMP, NFC, CAMERAS, INTERNET, REBOOT, RECOVERY, and VIBRATE, was giving false positive questions, as these words can be used anywhere. So, we manually checked and removed the not related questions. Additionally, we removed duplicate posts and posts with broken links. It resulted in 3447 questions in step \textcircled{7}. In step \textcircled{8}, we extracted the corresponding answer to the collected questions and got 3355 answers.

Then, we performed restriction and protection level classification and compared them with official documentation(\textcircled{9}). Finally, we performed qualitative analysis for categorization (\textcircled{10}) with questions and answers pair.  

\begin{figure}[h]
    \centering
    \includegraphics[width= 9 cm]{study1_methodology.jpg}
    \caption{Study Design for Investigating the Android Permission Related Challenges}
    \label{fig:studydesign}
\end{figure}

\subsection{ Data Analysis}

To address RQ1, we undertook a three-step process: Firstly, we identified all unique permissions that were referenced in the questions and answers of our data set. After this identification process, we proceeded to pair these permissions with their respective restriction types for Android 10, 11, 12, and 13 and protection level using the data collected in Step \textcircled{3}.

In the second part of our analysis, we examined how these restriction types changed over time, effectively determining if they evolved or remained the same across different Android versions. We tallied the number of questions and answers that discussed evolving permissions and those that dealt with non-evolving permissions. The analysis is summarized in Table ~\ref{table:permissionevolution}.

Lastly, in the third part, we found single question or answer could mention several permissions. Therefore, we tallied the total number of permissions mentioned on Stack Overflow (SO), which we designated as \textit{permission instances}.
We manually identified the Android version, if mentioned within a question or answer. We then analyzed the number of permission instances for each restriction type and protection level. If a particular Android version was specified in a question or answer, we used the restriction type for that version for the permission mentioned. In some cases, a question or answer might refer to a permission for a specific Android version, but we couldn't find that permission in the corresponding permission list for that version. We labeled these instances as \textit{mismatched}. The analysis is summarized in Table ~\ref{table:permissionrestriction} and Table ~\ref{table:permissionprotection}

\begin{table}[]
\scalebox{0.7}{
\begin{tabular}{lrrrr}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Evolution\\ Criteria\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{Questions}} &
  \multicolumn{2}{c}{\textbf{Answers}} \\
 &
  \multicolumn{1}{c}{\#Unique Permissions} &
  \multicolumn{1}{c}{\#Questions} &
  \multicolumn{1}{c}{\#Unique Permissions} &
  \multicolumn{1}{c}{\#Answers} \\ \hline
Non-Evolving      & 188 & 2811 & 121 & 1251 \\
Evolving  & 11  & 29   & 7   & 15   \\
No Permission & -   & 607  & -   & 2092 \\
Total         & 199 & 3447 & 129 & 3358 \\ \hline
\end{tabular}}
\caption{Question, Answer , and Permission summary with respect to Evolution}
\label{table:permissionevolution} 
\end{table}

\begin{table}[]
\begin{tabular}{lrr}
\hline
Restriction Type                                                  & \multicolumn{1}{l}{Question} & \multicolumn{1}{l}{Answer} \\ \hline
\begin{tabular}[c]{@{}l@{}}\#Public\\ API\end{tabular}            & 5494                         & 2028                       \\
\#Whitelisted                                                     & 157                          & 29                         \\
\begin{tabular}[c]{@{}l@{}}\#Greylist-max-o\end{tabular} & 114                          & 24                         \\
\#BlockList                                                        & 1                            & 1                          \\
\#Unsupported                                                     & 0                            & 0                          \\
\#Mismatched                                                      & 51                           & 57                         \\
Total                                                             & 5817                         & 2139                       \\ \hline
\end{tabular}
\caption{Restriction Type of the Permission Instances}
\label{table:permissionrestriction} 
\end{table}


\begin{table}[]
\begin{tabular}{lrr}
\hline
Protection Level                                                  & \multicolumn{1}{l}{Question} & \multicolumn{1}{l}{Answer} \\ \hline
\#Signature                                                       & 573                          & 167                        \\
\#Normal                                                          & 1491                         & 339                        \\
\#Dangerous                                                       & 3379                         & 1520                       \\
\begin{tabular}[c]{@{}l@{}}\#Signature\\ |Privileged\end{tabular} & 336                          & 97                         \\
\#Mismatched                                                      & 38                           & 16                         \\
Total                                                             & 5817                         & 2139                       \\ \hline
\end{tabular}
\caption{Protection Level of the Permission Instances}
\label{table:permissionprotection} 
\end{table}

To address RQ2, the 3447 questions were analyzed in two steps. First, we performed open coding to identify the themes, patterns, and concepts. Open coding is a qualitative research method used to analyze data in an exploratory and iterative way ~\cite{glaser2016open}. Second, based on the findings from open coding, we categorized the challenges faced by developers. One author performed open coding on the 3447 questions. They went through the dataset, identifying patterns, and assigned codes to represent the concepts that emerged from the data. Another author then participated in a verification process. They independently reviewed the sample of the coded data to ensure the codes accurately reflected the data. Any discrepancies or differences in coding were discussed and resolved through a consensus-building process. This verification step helped to increase the reliability and validity of the analysis, as it ensured that the coding process was consistent and reliable across all coders. This qualitative analysis derived five main categories: \textit{Implementation, Debugging, Conceptual Understanding, Documentation / Learning Resources, and Dependencies}. These were further divided into subcategories as in Figure~\ref{fig:classification_questions}. We provided descriptions and examples for all categories in the replication package\footnote{replication}. We also noticed that each question has two scenarios: either it had answers to the challenge mentioned in it or no answer. The questions have answers and scenarios: either it had an accepted answer or no accepted answer. Accepting an answer means that the author received an answer that worked for them personally \footnote{ https://stackoverflow.com/help/accepted-answer}. 

\begin{figure*}[h]
    \centering
    \includegraphics[width= 17 cm]{categorigation_question_study_01.png}
    \caption{Categorization of Questions Corresponding to Challenges (WS= With Solution, W/OS = Without Solution, AA = Accepted Answer)}
    \label{fig:classification_questions}
\end{figure*}

To address RQ3, similar to the analysis of RQ2, we used open coding and grouped the 3358 answers into five major categories: \textit{Implementation Guideline, Configuration Guideline, Documentation / Learning Resources, Conceptual Understating, and Debugging Steps}, summarized in  Figure ~\ref{fig:classification_answers}. Then we mapped the questions and answers categories, summarized in Table ~\ref{table:mapping} 

\begin{figure}[h]
    \centering
    \includegraphics[width= 8.5 cm]{categorigation_answer_study_1.png}
    \caption{Categorization of Answers Corresponding to Provided Solutions }
    \label{fig:classification_answers}
\end{figure} 

\begin{table}[H]
\scalebox{0.65}{
\begin{tabular}{lrrrrr}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Questions' \\ Categories\end{tabular}} & \multicolumn{5}{c}{\#Answers} \\ \cline{2-6} 
 &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Implementation \\ Guideline\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Configuration \\ Guideline\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Referred \\ Documentation\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Conceptual \\ Understanding\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Debugging \\ Steps\end{tabular}} \\ \hline
Implementation                                                                    & 602   & 165 & 59  & 146 & 4   \\
Debugging                                                                         & 1011  & 363 & 98  & 163 & 151 \\
\begin{tabular}[c]{@{}l@{}}Conceptual \\ Understanding\end{tabular}               & 81    & 40  & 35  & 108 & 4   \\
Documentation                                                                     & 20    & 8   & 14  & 8   & -   \\
Dependencies                                                                      & 134   & 86  & 15  & 27  & 15  \\
Total                                                                             & 1832  & 662 & 221 & 452 & 174 \\ \hline
\end{tabular}}
\caption{\label{table:mapping} Mapping of Questions' and Answers' Categories}
\end{table}

To address RQ4, we manually investigate if the questions and answers mention the restriction type and the protection level of the permissions. Lastly, we compare whether the information provided in the questions and answers matches the androids' official information. The comparison is summarized in Table ~\ref{table:restriction_comparison} and  Table ~\ref{table:Protection_comparison}).


\begin{table*}[]
\begin{tabular}{lrrrrrrrr}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Restriction\\ Type\end{tabular}}} & \multicolumn{4}{c|}{Question} & \multicolumn{4}{c}{Answer} \\ \cline{2-9} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Mentioned\\ Restriction \\ Type\end{tabular}} &
  \multicolumn{1}{c}{\# Matched} &
  \multicolumn{1}{c}{\#Unmatched} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# No \\ Permission\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Mentioned\\ Restriction\\ Type\end{tabular}} &
  \multicolumn{1}{c}{\# Matched} &
  \multicolumn{1}{c}{\# Unmatched} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# No \\ Permission\end{tabular}} \\ \hline
SDK                                                                                             & 22     & 16    & 2     & 4    & 18    & 11    & -    & 7   \\
Blocklist                                                                                       & 4      & -     & 4     & -    & 1     & -     & -    & 1   \\
Greylist-max-x                                                                                  & 4      & -     & 4     & -    & -     & -     & -    & -   \\
Unsupported                                                                                     & 3      & -     & 3     & -    & -     & -     & -    & -   \\
Total                                                                                           & 33     & 16    & 12    & 4    & 19    & 11    & -    & 8   \\ \hline
\end{tabular}
\caption{\label{table:restriction_comparison} Comparison between Community Provided Information and Official Information about Restriction Type}
\end{table*}



\begin{table*}[]
\begin{tabular}{lrrrrrrrr}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Protection\\ Level\end{tabular}}} & \multicolumn{4}{c|}{Question} & \multicolumn{4}{c}{Answer} \\ \cline{2-9} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Mentioned\\ Protection Level\end{tabular}} &
  \multicolumn{1}{c}{\# Matched} &
  \multicolumn{1}{c}{\# Unmatched} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# No \\ Permission\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Mentioned\\ Protection Level\end{tabular}} &
  \multicolumn{1}{c}{\# Matched} &
  \multicolumn{1}{c}{\# Unmatched} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# No \\ Permission\end{tabular}} \\ \hline
Dangerous                                                                                       & 69     & 41     & 18   & 10   & 77    & 14   & 15   & 18   \\
Normal                                                                                          & 46     & 29     & 13   & 4    & 39    & 28   & 6    & 5    \\
Signature                                                                                       & 72     & 42     & 14   & 16   & 44    & 20   & 9    & 14   \\
Total                                                                                           & 187    & 112    & 45   & 30   & 160   & 62   & 30   & 37   \\ \hline
\end{tabular}
\caption{\label{table:Protection_comparison} Comparison between Community Provided Information and Official Information about Protection Level}
\end{table*}


\begin{table}[]
\begin{tabular}{lrrrr}
\hline
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Developers'\\ Characteristics\end{tabular}} &
  \multicolumn{1}{c}{Question} &
  \multicolumn{1}{c}{Answer} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Accepted   \\ Answer\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Negative   \\ Answer\end{tabular}} \\ \hline
Reputation &
  18444.737 &
  42306.182 &
  62316.078 &
  14302.008 \\
SO   profile age &
  6.38 years &
  7.24 years &
  7.45 years &
  5.21 years \\ \hline
\end{tabular}
\caption{\label{table:Developers_characteristics} Mapping of Questions' and Answers' Categories}
\end{table}


\section{Results}

\subsection{Results of RQ1} From Table ~\ref{table:permissionevolution}, we can see among 766 permissions, only 188 unique permissions were discussed in the questions, and 129 unique permissions were discussed in the answers. For questions, 94.1\% of permissions are non-evolving, and for answers, 93.7\% of permissions are non-evolving. Similarly, most of the questions (81.5\%) and answers (37.19\%) discussed non-evolving permissions. In addition, we found that 607 questions and 2092 answers did not mention any specific permissions. 
In Table ~\ref{table:permissionrestriction}, developers discussed 5817 permission instances in the questions. Among them, 94.4\% of permission instances were Public-API. There were 51 mismatched permission instances, as those permissions were absent in the Android version mentioned in the questions. In the answers, developers mentioned permissions 2139 times, and 2028 were Public-API. For the answers, the number of mismatched permission was 57. 

From Table  ~\ref{table:permissionprotection}, we get the result about the protection level. Dangerous types of permissions were mostly discussed for both questions and answers. There were 38 and 16 mismatched permission instances in questions and answers, respectively, as those permissions were absent in the Android source code.

\begin{tcolorbox}
\textit{Summary RQ1: Our analysis found that developers face problems mostly related to non-evolving Public-API permissions. In terms of protection level, they face most problems with Dangerous level permissions. In some cases, they discuss permissions not present in the mentioned version or Android source code.}
\end{tcolorbox}


\subsection{ Results of RQ2}The five main categories for the developers' challenges are depicted in Figure ~\ref{fig:classification_questions} and reported next.

\subsubsection{Debugging} 
Debugging is finding and resolving errors or bugs in computer software. The posts discuss the concepts that have been coded but do not work. Most questions fall in the \textit {Debugging} category (1756). Among these 1756 questions, 69.1\% have answers, and only 31.03\% have accepted answers. These questions were divided into two subcategories, and one subcategory was further divided into three sub-subcategories : 

\textbf{Functional Improvement:} The questions refer to the process in which a developer aims to identify and rectify a faulty implementation that lacks an obvious error message and whose actual performance differs from the expected performance. 214 questions were related to this subcategory, where 151 of them have answers, and 63 of them did not have any answers. 

\textbf{Error Handling:} The questions where the developer wants to fix an implementation with an obvious error message. We categorized 1542 questions in this subcategory, where 1076 of them have answers, and 466 of them do not have any answers. We further divided this subcategory into three categories. 

  \begin{itemize}
    \item \textbf{Absence of Required Permission:} These questions are related to errors that occurred due to missing required permission. Among 1542 questions, 677 were related to this sub-subcategory, and 33\% of the questions (210) did have answers.

    \item \textbf{Sensitive or Restricted Permission Usage:}  Sensitive or Restricted Permission Usage is a situation that arises when an Android app is rejected or encounters errors due to its request for certain sensitive permissions. These permissions, according to Google, might be unnecessary or inappropriate for the app's functionality, or need to explain privacy policy. Only 182 questions were related to this category and 132 have answers. 
    
    \item \textbf{Exception or Warning:} The posts refer to any specific exception, warning, or error message other than sensitive permission usage and the absence of required permissions. The highest number of \textit{Error Handing} related questions (683) fall into this sub-subcategory. 470 of these questions have answers, whereas 213 do not have any. 
    \end{itemize}

\subsubsection{Implementation} 
The questions discuss aspects of not knowing how to implement something. The second highest number of questions falls in the \textit {Implementation} category (1056). Among these 1056 questions, 64.39\% have answers, and only 27.1\% have accepted answers. These questions were further divided into two subcategories: 

\textbf{Functionality Implementation:} The questions where developer wants to implement specific functionality. 805 questions were related to this subcategory, where 558 of them had answers, and 286 of them did not have any answers. 

\textbf{Alternative Solution or Best Practices:} The questions discuss aspects related to more optimal, secured solutions and aspects that the developer wants to find an alternative to an existing solution. 252 questions were related to this subcategory, where 162 of them had answers, and 90 of them did not have any answers. 


\subsubsection{Conceptual Understating} 
Questions aimed at understanding the inner workings principles behind a concept or technology. For our categorization, we only aimed at those questions which aimed at understanding Android permission-related concepts. 281 questions fall in this category. Among these 281 questions, 68.68\% have answers, and only 36.29\% have accepted answers. These questions were further divided into two subcategories: 

\textbf{Rationale Analysis:} The developer wants to understand the rationale behind a permission's behavior or behavioral changes. 130 questions were related to this subcategory, where 80 of them had answers, and 50 of them did not have any answers. 

\textbf{Permission Usage Learning:} The developer wants to learn how/when/where to use permission. 151 questions were related to this subcategory, where 113 of them had answers, and only 38 of them did not have any answers. 


\subsubsection{Documentation} 
The Android SDK documentation is extensive and a one-stop resource for complete information. Any questions related to documentation are categorized into this group. This category contains nine questions where 68.75\% have answers and  39.58\% have accepted answers. These questions were further divided into three subcategories: 

\textbf{Lack of Documentation:} The questions related to tutorials and documentation should cover parts of the Android Permissions in more detail.
24 questions were related to this subcategory, where 15 of them had answers, and the other nine did not have any answers. 

\textbf{Confusing Documentation:} The questions where the developers find such documentation challenging to understand, unclear, and incomplete descriptions.
17 questions are in this category; 12 has an answer, and the other five does not. 
    
\textbf{Contradictory Documentation:} The questions of a situation when various sources of the Android platform's documentation provide conflicting information about how to implement a particular feature or how a specific method, API, or permission acts. This category only has seven question, and three of them have the answer.

\subsubsection{Dependencies} 
The questions deal with issues depending on specific devices, specific versions, or other software dependencies. Eighteen questions fall into this category. Among these 306 questions, 60.78\% have answers, and only 27.77\% have accepted answers. These questions were further divided into four subcategories: 

\textbf{Version Dependency:} The developers are facing permission related issues for a specific Android version.
136 questions were related to this subcategory, where 95 of them have answers, and 41 of them do not have any answers. 
   
\textbf{Device Dependency:} The developers are facing permission related issues for a specific Android device. 103 questions were related to this subcategory, and almost 50\% (49) did not have answers. 
   
\textbf{Platform Dependency:} Developers are facing issues related to a specific platform. 16 questions were related to this subcategory, where nine of them have answers, and seven of them does not have any answers. This sub-sub category have lowest number of questions in this for this sub-category.
   
\textbf{Device and Version Dependency:} Developers are facing issues related to specific Android devices for specific Android versions. 51 questions were related to this subcategory, where 35 of them have answers, and 16 of them does not have any answers. 
   

\begin{tcolorbox}
Summary RQ2: Overall, we identified five core categories, 13 subcategories, and three sub-subcategories. Among 3447 questions, 66.78\% of them have answers, but only 30.02\% have accepted answers.
\end{tcolorbox}

\subsection{ Results of RQ3} For 3447 questions, 66.78\% of them have answers. In total, we got 3358 corresponding answers. We came up with five main categories for these answers, which is summarized in Figure ~\ref{fig:classification_answers} and also mapped with the questions' categories in Table ~\ref{table:mapping}

\textbf{Implementation Guideline:} The answers provide any guideline for implementing a functionality, improvement of functionality, or solution to errors, warnings, and exceptions. The highest number of answers (1849) are in this category. 602 of them were answered to \textit{Implementation} related questions, 1011 of them were answered for \textit{Debugging} related questions, 81 of them were answered for \textit{Conceptual Understanding} related questions, only 20 of them were answered for the \textit{Documentation} related questions, and 134 of them were answered to give implementation guideline when developers face \textit{Dependency} related problems.

\textbf{Configuration Guideline:} The answers provided a guideline for various parameters, options, and settings to have desired behavior and functionality. Only 662 answers are in this category. Among them, 165 were answering to \textit{Implementation} related question, 363 was for \textit{Debugging} related questions, and 40 were for \textit{Conceptual Understating}, only eight of them were answered for the \textit{Documentation} related and 86 were for \textit{Dependencies} related questions.

\textbf{Referred Documentation:} The answers where Android documentation and learning resources are referred to resolve issues. There are 221 answers in this category. Among them, 59 were answering to \textit{Implementation} related question, 98 was for \textit{Debugging} related questions, 35 for \textit{Conceptual Understating}, 14 for \textit{Documentation}, and 15 for \textit{Dependencies} related questions.

\textbf{Conceptual Understanding:} The answers explain the inner workings of principles and concepts of using permission. There are 452 answers in this category. Among them, 146 were answering to \textit{Implementation} related question, 163 was for \textit{Debugging} related questions, and 108 for \textit{Conceptual Understating}, eight answered the \textit{Documentation} related questions and 27 for \textit{Dependencies} related questions.

\textbf{Debugging Steps:} The answers explain the steps for debugging any situation. There are 174 answers in this category. Among them, four were answering to \textit{Implementation} related question, 151 was for \textit{Debugging} related questions, and four for \textit{Conceptual Understating}, and only 15 for \textit{Dependencies} related questions.


\begin{tcolorbox}
\textit{Summary RQ3: Our analysis uncovered five high-level categories for the answers to the questions. Highest 54.55\% of the answers fall into \textit{Implementation Guideline} category  whereas only 5.18\% of answers are in \textit{Configuration Guideline} category, which is the lowest.}
\end{tcolorbox}

\subsection{ Results of RQ4}
\textbf{Restriction Type Comparison with Androids' Official Information:} 
Only 22 Questions were mentioned about restriction type. In these questions they mentioned restriction type for 33 times. We compared the restriction type with Android's official information with respect to mentioned permissions in the questions. From Table ~\ref{table:restriction_comparison}, four questions did not mentioned any specific permissions and for the rest, 12 of these did not matched with the official restriction list which is 36.36\%. For the answers, only 17 answers mentioned about the restriction type for 19 times. 11 of these mentioned specific permissions and all of them matched with the official documentation and 8 of the questions did not mentioned any specific permissions , they only mentioned about different restriction type. Therefore, in the answers all of the permission instances' restriction type matched with the official information.
  
\textbf{Protection Level Comparison with Androids' Official Information:}
126 questions were mentioned about protection level which is a lot higher than restriction type. In these questions they mentioned protection level for 187 times. We compared these with Android's official information with respect to permissions. There are 30 questions where they did not mention any specific permission. From Table ~\ref{table:Protection_comparison}, we can  see 45 mentioned protection level did not matched with the official one which is 24.06\%. For the answers, 133 answers mentioned about the restriction type in total 160 times. Among these 37 did not have any specific permission. There are 62 (38.75\%) protection levels which matched with the official documentation of it's related permission. 

\begin{tcolorbox}
\textit{Summary RQ4: We found that developers are very unlikely to mention the restriction type, and protection level of the permissions. Even if they mentioned, the restriction type and protection level may not match with the official documentation. However, the information about protection level is more likely to match with the official documentation than restriction type.}
\end{tcolorbox}


==> rel_work_new.tex <==
\section{Related Work} 

Since its introduction in 2008, Android permissions system  has seen a significant research attention. One of the early security concerns that was raised by security community is overprivileged apps, a phenomenon referring to apps requesting unnecessary permissions (\cite{vidas2011curbing,felt2011android}). Noting that Android app developers should adhere to the principle of least privilege in their permission requests, \cite{felt2011android} developed Stowaway, a  tool for detection of excessive privileges in Android apps. Their analysis of 940 apps showed that roughly a third of these apps had more permissions than needed. A study of 30K Android apps from Google Play Store by \cite{taylorevolution2017} has further showed that free and popular apps are more likely to ask for additional permissions when they are being updated. 


%The recent study by~\cite{almomani2020comprehensive} confirmed They have also scrutinized the permissions framework through the lens of ten third-party and ten pre-installed  Android apps from 2016 to 2020. Remarkably, some apps experienced a 73.33\% surge in permission requests by 2020. 




To address this problem, several solutions aiming for automatic assessment of the requested permissions and their need for the app's functionality were proposed, e.g., 
Arcade (\cite{aafer2018precise}), Dynamo (\cite{Dawoud21}), PmDroid (\cite{gao2015}), IntentChecker (\cite{he2016detecting}), StaDART (\cite{ahmad2020stadart}). 



\subsection{Evolution of Android platform}
Android permission system has significantly evolved since its initial inception and   restricted the permission system by introducing safeguards
on non-SDK interfaces to regulate access to the Android platform



\cite{felt2011android}'s analysis revealed that while developers aim to minimize permissions, they typically fail due to gaps in API documentation. Indeed, gaps in Android permission documentation led to development of PScout, a static analysis tool for automatic extraction of permission specifications directly from the Android platform source code (\cite{au2012pscout}).




\cite{li2016accessing} empirically investigated 17 releases of the Android framework source code base to find the evolution of Android internal APIs and  APIs from three aspects: significance, impact, and adoption. They found that non-SDK APIs are commonly implemented in the Android framework, and a small set of non-SDK APIs can eventually become SDK APIs. However, most of them are removed during evolution. This study was based on early versions of Android ($\leq 6.0 $ ) before Google deployed the restriction on non-SDK APIs. In addition to that, their analysis may have false positive or false negative results as Google did not provide the complete list of non-SDK APIs at each API level at the time of their study. As a result, their findings need to be updated to reflect the current status of non-SDK APIs. Then,~\cite{li2020cda} performed an exploratory study of deprecated Android APIs from 377,474 commits from the GitHub repository of the Android framework and a set of randomly selected 10,000 Android apps from the official Google Play and 
third-party markets (NGPlay). They provided a research-based prototype tool called CDA and used it to mine different revisions of the Android framework code for characterizing deprecated APIs. With this mined data, they performed an empirical study to find the prevalence of deprecated APIs, their annotations and documentation, their removal and consequences, their replacement messages, developer reactions to API deprecation, and the evolution of the usage of deprecated APIs. Their results identified three bugs related to deprecated APIs. These bugs have been quickly assigned and positively appreciated by the framework maintainers, who claim these issues will be updated in future releases.




-----

\subsection{Android permission guidance on community platforms} The rapidly changing Android platform code, combined with a lack of documentation, prompted a significant increase in the number of developers seeking assistance within the community platforms.


There are also few studies related to effect of Android permissions' evolution on developers' community platform, (\cite{villanes2017software}, \cite{ajam2020api}). 
To understand the misuse of permissions, \cite{stevens2013asking} analyzed 10,000 free Android apps. They identified a substantial sub-linear correlation between how often a permission is used and its misuse rate. Furthermore, they investigated the connection between permission usage and related queries on StackOverflow and found that the popularity of permission is strongly associated with its misuse. They also investigated   Stack Overflow data and found that more widely used permissions get mentioned more often in questions on Stack Overflow.



\cite{linares2013api} analyzed the relationships among the API change, the fault-proneness of those APIs, and the success of the Android apps using those APIs. They have studied 7,097 Android apps and user ratings to determine how the change and fault proneness relate to applications' success. They provided insights that less usage of fault- and change-prone APIs contribute more to apps' successes. 

\cite{mcdonnell2013empirical} performed an in-depth case study on active open-source Android applications from GitHub, which have over 1000 commits, five or more authors, 100 or more line changes per commit, and at least one commit made in 2012. They analyzed the co-evolution behavior of Android API and dependent applications using the version history data found in GitHub. They found that API is evolving fast, with an average rate of 115 API updates per month, but client adoption needs to catch up with this pace of evolution. In addition to that,  clients use fast-evolving APIs are used more than slow-evolving APIs. Lastly, they found that the API usage adaptation code is more defect-prone than the one without API usage adaptation which indicate that developers avoid API instability. 

\cite{liu2021identifying} performed an empirical study on 1,000 real-world Android apps across 10 versions of the Android APIs to find the characteristics of Silently-Evolved Methods (SEM) whose behavior might have changed. Their results showed that SEMs exist in the Android API, and 957 apps used at least one SEM among their studied 1,000 apps. The corresponding documentation still needed to change accordingly. Because app developers rely on the provided documentation to evolve their apps, changes to methods that are not suitably documented may lead to unexpected failures in the apps using these methods.

To facilitate analysis of the correlation between permission and code smells, developers, conducting permission-related tasks,~\cite{Scoccia19},  recognized a significant gap in available resources and set out to bridge this gap by crafting a comprehensive dataset centered around permission-based changes and issues in open-source Android applications. To facilitate this research area, they aggregated data from an impressive 2,002 apps, involving contributions from a vast pool of 10,601 individual committers, cumulating a total of 789,577 commits. The methodology adopted by the authors entailed meticulous mining of app repositories from F-Droid. The extraction of the version followed this and commit histories and a subsequent analysis using a pair of permission analysis tools. The culmination of their effort serves as a valuable groundwork for potential future endeavors aiming to delve deeper into the intricacies of permission decisions and associated errors.

\cite{bagheri2018formal} analyzed the evolving Android permission protocol. They propose a formal model Android permission protocol using Alloy. They aimed to uncover potential lapses in this protocol through an entirely automated procedure. Their assertions were further fortified by investigating real-world Android applications. The empirical data underscored the gravity of the detected protocol vulnerabilities, suggesting that attackers might evade the permission checks entirely in some scenarios.

\cite{guerra2023leveraging} highlighted that addressing concept drift allows permissions to underpin robust and enduring malware detection tools. They evaluated the differentiating potential of various feature sets. Their findings reveal that the original permissions from Android 1.0 (API level 1) can effectively drive a detection model, yielding an impressive 0.93 F1 score over seven years of data. Additionally, they delved into the progression of permissions through both localized and overarching analytical techniques. 



\cite{aafer2018precise} introduced a method to accurately derive Android protection specifications in a path-sensitive manner using a unique graph abstraction technique. This is achieved through a tool named Arcade.
Arcade created a control flow graph from each public Android API and then converted this into an Access-control Flow Graph (AFG), which filters out non-relevant data while retaining the original control flow. This AFG is then processed to pull out access control conditions and their correlations, represented as a first-order logic formula. This formula-based map is then used to address overprivileged and component hijacking issues in Android apps.
Testing with four Android open-source projects' images indicated that Arcade's approach is pivotal, as around 41\% of API protections can not be correctly represented without it. Compared to the widely recognized Axplorer (\cite{backes2016demystifying}) method, Arcade detected 43\% more unnecessary permissions and reduced false positives in component hijacking detection by an average of 11 components per image. \cite{backes2016demystifying} analyzed the application framework, shedding light on previously unexplored areas. The study introduced an unprecedented classification of the framework's protected resources by creating a static runtime model. It also highlighted unique design patterns within the framework, notably different from those at the application level.
They adopted a top-down static analysis technique to face the hurdle of limited knowledge about the framework's core mechanisms. This approach was geared towards comprehensively understanding the framework's primary access points and meticulously navigating its control and data pathways, all with a keen eye on security and privacy. A notable divergence in design patterns between the framework and application layer posed challenges. To overcome this, a specialized static analysis method was crafted, resulting in a comprehensive understanding of the application framework.
Leveraging this deepened understanding, and the Axplorer tool was conceived to scrutinize the Android application framework. Trialed across four diverse Android iterations, Axplorer demonstrated its capability to streamline certain analyses by as much as 75\% without compromising on precision.



\cite{gao2015} presented PmDroid, a tool designed to safeguard data that falls outside the permissible boundaries of advertising networks. PmDroid is operated by preventing data transmission to advertising servers when a permission breach is detected within these networks. The researchers leveraged PmDroid to gauge the magnitude of permission violations within advertising networks.
For the purpose of this study, 53 prototype applications were developed, each incorporating a singular ad network library. These applications were endowed with the full spectrum of permissions available in Android 4.3. The team then monitored the data these apps transmitted over the internet. The study expanded its scope to scrutinize 430 apps available in the market. Throughout the research, a total of 76 distinct ad networks were unearthed.
A notable aspect of this research involved contrasting the permissions accessed by these ad networks against their official documentation. The findings of the study underscored a pressing concern: permission violations within ad networks are not merely hypothetical but a tangible issue in current advertising network ecosystems.


\cite{he2016detecting} introduced IntentChecker, a pioneering tool poised to detect and rectify permission leakage through an innovative lightweight mechanism. IntentChecker fortifies defenses against these leakages by introducing an authorization additional to the Inter Component Communication (ICC) framework and ingeniously auto-generates patches for apps identified as susceptible. For testing, they used two benchmarks: Droidbench and ICCbench, and a vast array of 4031 real-world applications, IntentChecker pinpointed 324 apps with discernible permission leakage. To further ascertain the robustness of its defense strategy, a random selection of 10 vulnerable apps was subjected to its mechanism. The results affirmed IntentChecker's prowess in curbing inter-app permission leakages.



\cite{Dawoud21} presented Dynamo, a dynamic testing tool designed to analyze Android's application framework security policy and validate static analysis tools' results. Their analysis of the permission revealed that five sensitive APIs are unprotected and 65 APIs with permission misconfigurations. In addition to that, they also found incomplete documentation for 66 APIs and imprecise for 9 APIs, which they reported to Google for corrective actions.

\cite{ahmad2020stadart}  highlighted the limitations of current analytical tools when confronted with dynamic code updates. This was exemplified using their test applications, Reflection-Bench and InboxArchiver. Building on this foundation, the authors introduced StaDART, an innovative solution that marries static and dynamic analysis techniques to expose the covert behavior typical of malware. Intriguingly, StaDART employs a dynamic code interposition mechanism, leveraging a vtable tampering strategy for API hooking. This approach was commendably non-intrusive, sidestepping any need to alter the Android framework. The authors further bolstered the tool's operational efficiency by merging it with DroidBot (\cite{li2017droidbot}), a triggering mechanism, promising a more streamlined and autonomous operation. They presented a comprehensive evaluation of StaDART using a dataset of 2000 real-world apps, encompassing both legitimate and malware specimens. Their findings, particularly when coupled with the Reflection-Bench results, compellingly suggest StaDART's adeptness at detecting malevolent behaviors typically obscured by static analysis tools.


To reduce the misuse of permissions by users, \cite{wei2015claim} explored correlation between an app's description and its associated permissions. The primary objective is to devise a model that can anticipate the correct permissions an app might require, using solely its description. Validating their approach with apps sourced from the Google Play Market, they report an impressive prediction accuracy of up to 87\%. This suggests that, given a user's thorough comprehension of an app's description, the proposed model can function as a valuable alert mechanism. It can flag potential inconsistencies between the app's described functionality and its permission requests — a tactic frequently exploited by malicious software.

\cite{anwer2014chiromancer}  introduced a tool called Chiromancer, designed to manage an app's permissions with high precision and regulate the app's resource usage. Moreover, it is used for the optimization of an app's resource consumption tailored to individual preferences. This framework depends on static code analysis combined with code injection, and it operates on compiled code, eliminating the need for the app's source code. To substantiate their claims, the authors employed Chiromancer on publicly accessible applications from Google Play, enhancing their performance. A comparative assessment of energy and data usage, pre and post-code injection, demonstrated notable performance enhancements, underscored the tool's potential efficacy.
 

\cite{felt2011permission} discussed the concept of permission redelegation in Android OS, which undermines user approval requirements and can lead to potential security vulnerabilities. To address this issue, the authors introduce Inter Process Communication (IPC) inspection, a new mechanism that limits an app's permissions when it interacts with a less privileged one, demonstrating its effectiveness in preventing real-world attacks on Android apps.


\cite{barrera2010methodology} introduced an innovative approach to empirically examining permission-based security models. Central to this novel methodology is the utilization of the Self-Organizing Map (SOM) algorithm, as delineated by Kohonen. Even though the authors articulated a framework that holded potential applicability across a multitude of architectures, their research distinctly focused on a case study encompassing the analysis of 1,100 Android applications. Apart from its specific application in this context, the proposed methodology beckons interest as a visualization tool for permission-based systems that transcend the confines of the Android platform. 


\cite{yang2022demystifying} studied 200k Android apps and the source code of three Android versions to understand the present status of using non-SDK APIs, security bypass, and the evolution of non-SDK APIs. They constructed a dataset for APK used in their study, including benign and malicious apps. They also built an automated app scanner called veridex++ and generated the non-SDK API lists. After doing a multi-dimension analysis, they found that after Google launched its restriction for non-SDK APIs, access to those has stopped. However, still, they can be bypassed by destroying the integrity of the API caller's identity using double-reflection and call stack breaking. Then they found that using non-SDK APIs is very common even after Google launched the restriction. App developers are only interested in a small part of non-SDK APIs, and the purpose is to use unique features not supported by the SDK. In the security aspect, non-SDK APIs have been abused for malware to achieve malicious purposes. Even for the same APIs, the usages of malicious and benign apps are usually different. Lastly, they mentioned that the reasons for enhancing API restrictions are mainly for security concerns and fine-grained control, and loosening API restrictions is mainly due to developer requests and newly added features.

\cite{he2022systematic} studied the security for Android non-SDK service APIs and found that the security checks may be bypassed by directly exploiting the non-SDK APIs in the service helpers. This paper systematically studied the vulnerabilities due to the non-SDK API exploitation and analyzed the effectiveness of Google's countermeasures. Their goal was to find out if there are still vulnerable hidden APIs that can be exploited in the newest Android 12. To address their goal, they have developed a static analysis tool called ServiceAudit to automatically mine the inconsistent security enforcement between service helper classes and the non-SDK service APIs. They applied ServiceAudit to Android 6 to 12 and discovered 112 vulnerabilities in Android 6 with 84.2\% accuracy. Moreover, Android 11 and 12 identified more than 25 non-SDK APIs with inconsistent protections. They found that none of the vulnerable APIs can work on Android 12, but one vulnerable API called `requestPinShortcut' could lead to severe security problems in Android 11.

\cite{cai2019large} undertook an extensive longitudinal analysis of compatibility issues within 62,894 benign applications developed over eight years. They investigated the symptoms and causative factors behind these incompatibility issues. Their investigation also encompassed actual runtime incompatibilities by examining system logs and execution traces of 15,045 applications. They found that, the omnipresence and persistence of compatibility issues at both installation and runtime phases, with the latter displaying a higher frequency. Interestingly, they noted that specific Android versions did not exhibit consistent patterns of increased or decreased app incompatibilities. Their analyses found that installation-time incompatibilities were intrinsically linked to the minSdkVersion cited in applications. At the same time, runtime discrepancies had a stronger association with the API level of the base platform. They attributed the majority of installation-time incompatibilities to the integration of native libraries that were not architecturally aligned. In contrast, runtime incompatibilities stemmed mainly from the evolution and changes in the SDK's API. The authors graciously provided a deeper understanding of these app incompatibilities and proposed valuable advice for both the Android app developers and their users to mitigate these issues.

\cite{wei2016taming} characterized the symptoms and root causes of compatibility issues in Android apps and disclosed that the patches of these issues exhibit common patterns. After that, they propose a technique named FicFinder to automatically detect and capture Android APIs and their associated context by which compatibility issues are triggered. They evaluated FicFinder with 27 large-scale open-source Android apps and found that FicFinder can precisely detect compatibility issues in these apps and uncover previously-unknown issues. Their results indicated that API evolution causes compatibility issues in Android apps. 

~\cite{li2018cid} introduced CiD, an innovative automated methodology designed to systematically model the lifecycle of Android APIs and assess app bytecode. This analysis is critical as it flags potential compatibility issues that may arise. The authors undertook an exhaustive evaluation of all API versions by analyzing the source code of the Android framework. They meticulously extracted all public API methods and accounted for over 300 recorded releases on the Android code base repository at the time of their study. Given that multiple releases can be tied to a single API level due to minimal impactful changes, they concentrated on one release per API level. Their assessment spanned 24 releases covering API levels 1 through 25, offering a detailed mapping between each API level and its associated public APIs. Through hands-on application, the authors demonstrated the utility of CiD, showing its capability to assist developers in rectifying their apps. Remarkably, CiD outperformed existing state-of-the-art methods in benchmark app testing, emphasizing its efficacy in addressing numerous challenges tied to automatic detection.

To mitigate compatibility issues~\cite{scalabrino2019data} introduced an alternative of CiD named ACRYL, a data-driven methodology that learns from modifications made in other applications due to API changes. ACRYL learns from the insights by studying modifications made to various apps as a reaction to API alterations, a strategy they refer to as client side learning. Such an approach empowers ACRYL with a twofold capability: detecting compatibility challenges and proffering potential solutions.
In an attempt to evaluate the efficacy of ACRYL, the authors compared it with CiD tool. Intriguingly, their empirical findings highlighted that neither tool could be decisively deemed superior. The strength of both methodologies lies in their complementarity. Remarkably, the sets of API compatibility issues each tool identified exhibited minimal overlap. Such observations lead to an intriguing proposition: there might be substantial merit in amalgamating both tools, leveraging their collective might to extract rules for issue detection and resolution from both the API and its clients.


\cite{he2018understanding} undertook a empirical investigation across 11 distinct Android versions, evaluating a significant sample of 4,936 Android apps. Their findings shed light on the marked API alterations between successive Android versions. On average, each release introduces 140.8 new types, 1,505.6 new methods, and 979.2 new fields. Interestingly, the Android Support Library, an integral component of the Android OS, only encapsulates less than 23\% of these newly introduced methods and even fewer new types and fields. Such a disparity necessitates additional coding by app developers to ensure compatibility across diverse OS versions, with 91.84\% of Android apps resorting to this approach. The authors observed that 88.65\% of these compatibility-centric codes bear a recognizable pattern, relying on the android.os.Build.VERSION.SDK\_INT variable. Emerging from these insights, the authors introduced IctApiFinder, a novel tool designed to identify incompatible API usages within Android applications. This tool, leveraging an inter-procedural data-flow analysis framework, adeptly calculates the OS versions where a specific API might be summoned. Their examination of 1,425 apps pinpointed incompatible API usage in 361 of them. A comparative analysis with Android Lint affirmed the superiority of IctApiFinder, which guarantees sound results and diminishes false positives by a substantial 82.1\%. It is worth noting that upon notifying 13 app developers of the discovered issues, five confirmations and three subsequent fixes have been reported.

\cite{huang2018understanding} the authors address a particularly nuanced set of callback compatibility issues within the Android framework. While updates to the Android framework are frequently discussed, there is a gap in understanding their ramifications on app control flows and the resulting callback compatibility issues. To delve deeper into this, the authors examined Android documentation and also embarked on an empirical study focusing on 100 real-world instances of such issues, aiming to decode the interplay between callback API evolutions and the genesis of these compatibility challenges. Drawing insights from this empirical analysis, they introduced a novel graph-based model to articulate the inconsistencies in control flow birthed by API evolutions. Building on this, they put forth a static analysis mechanism, aptly named Cider, envisioned to pinpoint callback compatibility issues precisely. This technique was evaluated on a set of 20 widely-used open-source Android apps. Cider's effectiveness was evident as it unearthed 13 previously unidentified callback compatibility challenges, of which developers validated 12, and 9 have already been rectified.

\cite{mahmud2021android}  introduce ACID, designed to unearth compatibility challenges arising from the evolution of APIs. The core of this approach was related to discerning API variations and subsequently employing static analysis on Android apps' source code. This dual-pronged method equipped ACID to identify the usual API invocation compatibility issues and the often overlooked API callback compatibility problems.
To validate ACID's effectiveness, the authors evaluated it against the current best-in-class methodologies using 20 benchmark apps from prior research as the testing ground. The findings were noteworthy: ACID demonstrated superior precision and showcased expedited detection speeds. Further emphasizing its real-world relevance, the team extended their evaluation to encompass 35 real-world applications. This comprehensive analysis underscored ACID's potential as a robust solution in Android app development, especially in the context of API evolution-driven compatibility challenges.

The study by \cite{lee2023polyscope} aimed to shield Android and OEM services from potential threats posed by third-party apps. However, in an attempt to create standout features, OEMs sometimes introduce vulnerabilities because they mishandle this intricate web of policies. In their study, they introduced the POLYSCOPE tool. This tool investigated through the amalgamation of Android's filesystem access controls to pinpoint operations that adversaries might exploit for privilege escalation, termed as `attack operations'. Notably, POLYSCOPE factors in how attackers could tweak permissions to identify hidden attack routes. Through our research, we highlighted the potential of POLYSCOPE by evaluating Android's newly added Scoped Storage defense mechanism. Their findings showed that incorporating POLYSCOPE's analysis into a fresh policy is feasible if that policy solely tightens permissions – as is the case with Scoped Storage. Upon applying POLYSCOPE to multiple Android versions, including three from Google and five from OEMs, they found that Scoped Storage cuts the potential attack operations on external storage by over half. But, two new vulnerabilities surfaced due to the piecemeal adoption of Scoped Storage by OEMs. Hence, they further explored an optimal setting with POLYSCOPE where all applications fully align with Scoped Storage. In such a scenario, the number of dubious entities capable of initiating attack operations plummets by over 65\% on OEM systems. Conclusively, POLYSCOPE proves invaluable for Android OEMs, aiding them in navigating through intricate access controls to highlight specific attack avenues that warrant a closer look.


\cite{guerra2023rpcdroid} presented RPCDroid, a tool designed for dynamic analysis that actively monitors Android mobile applications' behavior, UI events and permissions when they access device resources that demand high-risk permissions. Their evaluation of RPCDroid showcased its capability to pinpoint different contexts under which the same sensitive resource is accessed. When they tested RPCDroid on a range of popular apps, it became evident that many apps frequently access identical resources but through varied user interactions.

\cite{xia2020android} presented the first extensive study exploring the management of evolution-induced API compatibility issues in approximately 300,000 Android market applications. More crucially, they investigated the corresponding solutions where applicable. They have explored diverse behaviors and various APIs.
The authors introduce RAPID, an innovative automated tool to support this large-scale analysis. RAPID is designed to determine the resolution status of a compatibility issue. It used static analysis and machine learning methodologies. The efficacy of the classifier used is highlighted by its impressive F1 scores: 95.21\% in the training phase and 91.96\% during validation.
RAPID's application to the study has led to several insightful revelations. For instance, it was observed that a mere 38.4\% of developers opted to offer alternative implementations when dealing with incompatible API invocations. Furthermore, the study underscored that developers often employ more varied and innovative strategies to rectify compatibility concerns than the recommendations set forth by Google. 

Android apps, popularly used for tasks like banking, social media, and shopping, often require permissions to access sensitive features, such as internet connectivity. Unfortunately, some apps exploit these permissions for malicious activities, including unauthorized data access and fraudulent credit card transactions. In response to this challenge, \cite{rubio2023dypoldroid} introduced DyPolDroid. It is a dynamic security framework integrated with Android Enterprise, allowing both users and administrators to implement 'Counter-Policies'. These are user-friendly tools designed to limit the permissions of potentially harmful apps, ensuring robust protection without needing intricate security knowledge. As part of their research, they developed Laverna, an app that showcases both proper and improper use of permissions. For transparency and to foster further research, they have made DyPolDroid and Laverna's source codes freely accessible to the public.

To identify information leaks in Android applications, current analysis techniques typically apply a two-level information flow policy, often missing the built-in permissions system of Android. This oversight can result in imprecise analysis outcomes. It is evident that integrating permissions can lead to a more detailed flow policy. \cite{liu2023permission} suggested a policy that includes permissions for secure information flow and provides a method to enforce it statically. They crafted a simplified language capturing Android's typical features, base our security policy on a subset of permissions, and establish rules to ensure the security of data flows. Additionally, they created a mechanism that can pinpoint potential insecure data flows by evaluating program components. To underscore their policy's practicality, they explored two common security threats and demonstrate how our framework can detect such vulnerabilities. Their tests confirmed their method's efficiency and scalability for genuine apps.

\subsection{Android permission and Developers Community Platforms}

Linares-V{\'a}squez et al. investigated a relationship between
API changes and developers' reactions (\cite{linares2014api}). They investigated 213,836 Android-related questions from Stack Overflow till August 2012. Their findings suggested that when the behavior of APIs is modified, the Android developers usually have more questions. In addition, they found that deleting public methods from APIs is a trigger question with two types of characteristics (i) more discussed and of major interest to the community, and (ii) posted by more experienced developers.

\cite{ajam2020api} explored the landscape of API topic issues as they appear on Stack Overflow. By performing a methodical empirical analysis on a curated sample of 400 Q\&A threads, they endeavor to pinpoint the core issues related to APIs. Through a meticulous thematic analysis of this sample, the study unveils eight predominant topics concerning APIs. Notably, topics like API usage, debugging, API constraints, and API security stand out as the most prevalent concerns in the community. The paper further enriches the discussion by providing illustrative examples showcasing the variety of support extended by the SO community to address these topics. Furthermore, the authors thoughtfully delve into potential avenues to harness the insights garnered from this study. 

\cite{villanes2017software}  leveraged the extensive repository of Stack Overflow to conduct a rigorous analysis of the primary topics related to Android testing. By adeptly utilizing the Latent Dirichlet Allocation (LDA) algorithm, they have succinctly summarized queries about mobile testing. The research distinctly highlights that themes encompassing testing tools, functional testing, and unit testing feature more prominently in discussions compared to other areas.



\textbf{Summary} The previous research focused on compatibility issues, misuse of permissions, vulnerabilities related to permissions, and tools for resolving those challenges. Here only a few studies focused on the developers' perspective on permission-related issues. Though ~\cite{linares2014api} mentioned that developers have more questions when the API behavior is modified, they did not investigate what type of questions developers ask or the challenges developer face regarding permissions. Moreover, it is crucial to understand the challenges of permissions faced by developers to mitigate the misuse, and security risks in apps. Our study focuses on the permission-related developers' challenges and solutions provided by the community to bridge the knowledge gap. This will also provide the researcher insight into the Android permission-related challenges that need to be mitigated to reduce the misuse of Android permissions.


